The Supply of Motivated Beliefs

When people choose what messages to send to others, they often consider how others will interpret the messages. A sender may expect a receiver to engage in motivated reasoning, leading the receiver to trust good news more than bad news, relative to a Bayesian. This paper experimentally studies how motivated reasoning affects information transmission in political settings. Senders are randomly matched with receivers whose political party's stances happen to be aligned or misaligned with the truth, and either face incentives to be rated as truthful or face no incentives. Incentives to be rated as truthful cause senders to be less truthful; when incentivized, senders send false information to align messages with receivers' politically-motivated beliefs. The adverse effect of incentives is not appreciated by receivers, who rate senders in both conditions as being equally likely to be truthful. A complementary experiment further identifies senders' beliefs about receivers' motivated reasoning as the mechanism driving these results. Senders are additionally willing to pay to learn the politics of their receivers, and use this information to send more false messages.

==> 1_competition_noprior.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Vs. Party-True Aligned}         &\multicolumn{1}{c}{Vs. No Info}         &\multicolumn{1}{c}{Vs. Neutral Topics}         \\
\hline
Party-False Aligned &    0.024         &    0.017         &    0.041         \\
                    &  (0.026)         &  (0.028)         &  (0.026)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned\hspace{20mm} &$\checkmark$         &                  &                  \\
Vs. No Info         &                  &$\checkmark$         &                  \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         \\
\hline
Observations        &     5254         &     5137         &     4368         \\
Subjects            &      126         &      126         &      125         \\
Mean                &    0.228         &    0.239         &    0.224         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_incentives_effect.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\hline
Incentivized        &    0.072\sym{***}&    0.073\sym{***}&    0.109\sym{***}&    0.107\sym{***}&    0.050\sym{*}  &    0.051\sym{*}  \\
                    &  (0.026)         &  (0.026)         &  (0.037)         &  (0.037)         &  (0.029)         &  (0.028)         \\
Party-False Aligned &                  &                  &                  &                  &    0.061\sym{**} &    0.062\sym{**} \\
x Incentivized      &                  &                  &                  &                  &  (0.026)         &  (0.026)         \\
Party-False Aligned &                  &                  &                  &                  &   -0.005         &   -0.003         \\
x Unincentivized    &                  &                  &                  &                  &  (0.027)         &  (0.027)         \\
Question FE         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Subject controls    &                  &$\checkmark$         &                  &$\checkmark$         &                  &$\checkmark$         \\
All Questions       &$\checkmark$         &$\checkmark$         &                  &                  &$\checkmark$         &$\checkmark$         \\
Only Party-False Aligned &                  &                  &$\checkmark$         &$\checkmark$         &                  &                  \\
\hline
Observations        &    14248         &    14248         &     4702         &     4702         &    14248         &    14248         \\
Subjects            &      249         &      249         &      220         &      220         &      249         &      249         \\
Mean                &    0.250         &    0.250         &    0.272         &    0.272         &    0.250         &    0.250         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_incentivized_noprior.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Vs. Party-True Aligned}         &\multicolumn{1}{c}{Vs. No Info}         &\multicolumn{1}{c}{Vs. Neutral Topics}         &\multicolumn{1}{c}{Vs. All}         \\     
\hline
Party-False Aligned &    0.092\sym{***}&    0.075\sym{***}&    0.051\sym{*}  &    0.067\sym{***}\\
                    &  (0.028)         &  (0.023)         &  (0.028)         &  (0.020)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &     5486         &     4963         &     4313         &     9278         \\
Subjects            &      124         &      124         &      124         &      124         \\
Mean                &    0.296         &    0.303         &    0.327         &    0.292         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_incentivized_prior.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Vs. Party-True Aligned}         &\multicolumn{1}{c}{Vs. No Info}         &\multicolumn{1}{c}{Vs. Neutral Topics}         &\multicolumn{1}{c}{Vs. All}         \\
\hline
Party-False Aligned &    0.071\sym{**} &    0.072\sym{***}&    0.049\sym{*}  &    0.053\sym{**} \\
                    &  (0.032)         &  (0.023)         &  (0.029)         &  (0.021)         \\
Prior-False Aligned &    0.248\sym{***}&    0.229\sym{***}&    0.226\sym{***}&    0.216\sym{***}\\
                    &  (0.053)         &  (0.059)         &  (0.060)         &  (0.049)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &     4990         &     4705         &     4055         &     8782         \\
Subjects            &      124         &      123         &      124         &      124         \\
Mean                &    0.296         &    0.297         &    0.322         &    0.292         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_incentivized_prior_nolast.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Vs. Party-True Aligned}         &\multicolumn{1}{c}{Vs. No Info}         &\multicolumn{1}{c}{Vs. Neutral Topics}            \\
\hline
Party-False Aligned &    0.071\sym{**} &    0.072\sym{***}&    0.049\sym{*}   \\
                    &  (0.032)         &  (0.023)         &  (0.029)          \\
Prior-False Aligned &    0.248\sym{***}&    0.229\sym{***}&    0.226\sym{***} \\
                    &  (0.053)         &  (0.059)         &  (0.060)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                                   \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$           \\
Vs. Party-True Aligned &$\checkmark$         &                  &                      \\
Vs. No Info         &                  &$\checkmark$         &                    \\
Vs. Neutral Topics  &                  &                  &$\checkmark$              \\
\hline
Observations        &     4990         &     4705         &     4055        \\
Subjects            &      124         &      123         &      124         \\
Mean                &    0.296         &    0.297         &    0.322            \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_incentivized_prior_only50.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
Party-False Aligned &    0.101\sym{**} &    0.115\sym{**} &    0.172\sym{***}&    0.111\sym{***}\\
                    &  (0.049)         &  (0.045)         &  (0.045)         &  (0.036)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned\hspace{20mm} &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &      448         &      420         &      356         &      798         \\
Subjects            &      119         &      115         &      111         &      124         \\
Mean                &    0.272         &    0.255         &    0.295         &    0.247         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_incentivized_prior_slides.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Vs. Party-True Aligned}         &\multicolumn{1}{c}{Vs. No Info}         &\multicolumn{1}{c}{Vs. Neutral Topics}         &\multicolumn{1}{c}{Vs. All Others}         \\
\hline
Party-False Aligned &    0.071\sym{**} &    0.072\sym{***}&    0.049\sym{*}  &    0.053\sym{**} \\
                    &  (0.032)         &  (0.023)         &  (0.029)         &  (0.021)         \\
Prior-False Aligned &    0.248\sym{***}&    0.229\sym{***}&    0.226\sym{***}&    0.216\sym{***}\\
                    &  (0.053)         &  (0.059)         &  (0.060)         &  (0.049)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &     4990         &     4705         &     4055         &     8782         \\
Subjects            &      124         &      123         &      124         &      124         \\
Mean                &    0.296         &    0.297         &    0.322         &    0.292         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Subject-level clustered standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_unincentivized_noprior.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Vs. Party-True Aligned}         &\multicolumn{1}{c}{Vs. No Info}         &\multicolumn{1}{c}{Vs. Neutral Topics}         &\multicolumn{1}{c}{Vs. All Others}         \\
\hline
Party-False Aligned &    0.006         &   -0.034         &   -0.009         &   -0.003         \\
                    &  (0.028)         &  (0.030)         &  (0.024)         &  (0.021)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &     5136         &     4888         &     4189         &     9239         \\
Subjects            &      125         &      125         &      125         &      125         \\
Mean                &    0.212         &    0.215         &    0.204         &    0.210         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 1_unincentivized_prior.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Vs. Party-True Aligned}         &\multicolumn{1}{c}{Vs. No Info}         &\multicolumn{1}{c}{Vs. Neutral Topics}         &\multicolumn{1}{c}{Vs. All}         \\
\hline
Party-False Aligned &    0.005         &   -0.038         &   -0.011         &   -0.006         \\
                    &  (0.032)         &  (0.030)         &  (0.024)         &  (0.023)         \\
Prior-False Aligned &    0.063         &    0.074\sym{*}  &    0.071         &    0.054         \\
                    &  (0.039)         &  (0.040)         &  (0.045)         &  (0.034)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &     4636         &     4619         &     3920         &     8739         \\
Subjects            &      125         &      125         &      125         &      125         \\
Mean                &    0.211         &    0.215         &    0.203         &    0.209         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 2_incentives_effect.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\hline
Incentivized        &    0.081\sym{***}&    0.078\sym{***}&    0.172\sym{***}&    0.167\sym{***}&    0.037         &    0.035         \\
                    &  (0.023)         &  (0.022)         &  (0.036)         &  (0.036)         &  (0.025)         &  (0.025)         \\
Party-False Aligned &                  &                  &                  &                  &    0.136\sym{***}&    0.135\sym{***}\\
x Incentivized      &                  &                  &                  &                  &  (0.032)         &  (0.032)         \\
Party-False Aligned &                  &                  &                  &                  &    0.006         &    0.006         \\
x Unincentivized    &                  &                  &                  &                  &  (0.025)         &  (0.025)         \\
Question FE         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Subject controls    &                  &$\checkmark$         &                  &$\checkmark$         &                  &$\checkmark$         \\
All Questions       &$\checkmark$         &$\checkmark$         &                  &                  &$\checkmark$         &$\checkmark$         \\
Only Party-False Aligned &                  &                  &$\checkmark$         &$\checkmark$         &                  &                  \\
\hline
Observations        &     2421         &     2421         &      822         &      822         &     2421         &     2421         \\
Subjects            &      500         &      500         &      429         &      429         &      500         &      500         \\
Mean                &    0.274         &    0.274         &    0.318         &    0.318         &    0.274         &    0.274         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 2_incentivized.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
Party-False Aligned &    0.145\sym{***}&    0.098\sym{**} &    0.090\sym{**} &    0.100\sym{***}\\
                    &  (0.045)         &  (0.041)         &  (0.041)         &  (0.033)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned\hspace{20mm} &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &      779         &      789         &      638         &     1470         \\
Subjects            &      229         &      223         &      206         &      245         \\
Mean                &    0.336         &    0.335         &    0.352         &    0.307         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> 2_unincentivized.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
Party-False Aligned &   -0.022         &    0.025         &   -0.065\sym{*}  &   -0.009         \\
                    &  (0.028)         &  (0.034)         &  (0.033)         &  (0.024)         \\
Question FE         &$\checkmark$         &$\checkmark$         &                  &                  \\
Subject FE          &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Round FE            &$\checkmark$         &$\checkmark$         &$\checkmark$         &$\checkmark$         \\
Vs. Party-True Aligned\hspace{20mm} &$\checkmark$         &                  &                  &$\checkmark$         \\
Vs. No Info         &                  &$\checkmark$         &                  &$\checkmark$         \\
Vs. Neutral Topics  &                  &                  &$\checkmark$         &$\checkmark$         \\
\hline
Observations        &      803         &      812         &      695         &     1529         \\
Subjects            &      235         &      243         &      224         &      255         \\
Mean                &    0.241         &    0.230         &    0.253         &    0.243         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}

